A Generalized Grand-Reaction Method for Modelling the Exchange of Weak (Polyprotic) Acids between a Solution and a Weak Polyelectrolyte Phase

We introduce a Monte-Carlo method that allows for the simulation of a polymeric phase containing a weak polyelectrolyte, which is coupled to a reservoir at a fixed pH, salt concentration and total concentration of a weak polyprotic acid. The method generalizes the established Grand-Reaction Method by Landsgesell et al. [Macromolecules 53, 3007-3020 (2020)] and thus allows for the simulation of polyelectrolyte systems coupled to reservoirs with a more complex chemical composition. In order to set the required input parameters that correspond to a desired reservoir composition, we propose a generalization of the recently published chemical potential tuning algorithm of Miles et al. [Phys. Rev. E 105, 045311 (2022)]. To test the proposed tuning procedure, we perform extensive numerical tests for both ideal and interacting systems. Finally, as a showcase, we apply the method to a simple test system which consists of a weak polybase solution that is coupled to a reservoir containing a small diprotic acid. The complex interplay of the ionization various species, the electrostatic interactions and the partitioning of small ions leads to a non-monotonous, stepwise swelling behaviour of the weak polybase chains.

==> definitions.tex <==
% use only packages that we really need!

%\usepackage{fontenc}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}

%\usepackage{subfigure}
\usepackage{graphicx}
\graphicspath{{figures/}}
\usepackage{color}
\usepackage{units}
\usepackage{hyperref}
\hypersetup{colorlinks,%
           citecolor=blue,%
          filecolor=blue,%
           linkcolor=blue,%
           urlcolor=blue,%
       pdfborder=0 0 0}
%\usepackage[final]{hyperref}

\usepackage[table]{xcolor}
\usepackage[german,english]{babel}



\usepackage[version=3]{mhchem}
\usepackage[version=3]{mhchem} % Formula subscripts using \ce{}
\usepackage{chemfig} %chemical reactions
\usepackage[utf8]{inputenc}
\usepackage{csquotes}

\usepackage{placeins}
\usepackage{pdfpages}
\usepackage{listings}


% uncomment one(!) of the following lines to enable/disable todo boxes
%\usepackage[disable]{todonotes}
\usepackage[textsize=small]{todonotes}

\usepackage{tcolorbox}
\usepackage{xifthen}

\newcommand{\nbar}{\text{$\bar{n}$} }
\newcommand{\todoi}[1]{{\todo[inline]{#1}}}	%	for for personal notes
\newcommand{\todopH}[1]{{\todo[color=blue!40, author=Pascal, inline]{#1}}}	%	for for personal notes
\newcommand{\lyxdot}{.} % to be able to have dot "." in filenames
\newcommand{\PE}{polyelectrolyte} % to be able to have dot "." in filenames
\newcommand{\boxl}{box_l} % to be able to have dot "." in filenames
\newcommand*{\molperl}{\unit{mol\,dm^{-3}}}






\usepackage[utf8]{inputenc} %P:K to enable typesetting of my name and other names with diacritics
%\usepackage[T1]{fontenc}

\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
  frame=single,
  breaklines=true,
  postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space},
}

% Let's use author-year bibliography to help checking that we have the correct references.
% We can switch to the usual numbered style just before submission - simply uncomment the line below.
%\usepackage{natbib}
%\setcitestyle{authoryear,square}

%\newlength\plotwidth \setlength{\plotwidth}{0.63\textwidth}
\newlength\plotwidth%
%\setlength{\plotwidth}{3.25in} % the maximum figure width given by the author guidelines of Macromolecules 05/2015

\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\etal}{\emph{et al}}
\newcommand{\kb}{k_\mathrm{B}}
\newcommand{\lb}{\lambda_\mathrm{B}}
\newcommand{\ld}{\lambda_\mathrm{D}}
\newcommand{\lp}{l_\mathrm{p}}
\newcommand{\lB}{l_\mathrm{Bjerrum}}
\newcommand{\kT}{k_\mathrm{B}T}
\newcommand{\Rend}[0]{R_\mathrm{e}}
\newcommand{\Rg}{R_\mathrm{g}}
\newcommand{\Rout}[0]{R_\mathrm{out}}
\newcommand{\Rstar}{R_{\mathrm{star}}}
\newcommand{\Rbox}{R_{\mathrm{box}}}
\newcommand{\Rmax}{R_{\mathrm{max}}}
\newcommand{\Ro}{R_\mathrm{0}}
\newcommand{\Fpo}{F^\mathrm{po}}
\newcommand{\avg}[1]{\left<{#1}\right>}
\newcommand{\lan}{{\cal{L}}}
\newcommand{\ilan}{{\cal{L}}^{-1}}

\newcommand{\muref}{\mu^{\ominus}}
\newcommand{\muid}{\mu^\mathrm{id}}
\newcommand{\muex}{\mu^\mathrm{ex}}
\newcommand{\musalt}{\mu_\mathrm{s}}
\newcommand{\cs}{c_\mathrm{salt}}
\newcommand{\cpoly}{c_\mathrm{0}}
\newcommand{\co}{c_{0}}
\newcommand{\ccat}{c_{\mathrm{cat}}}
\newcommand{\can}{c_{\mathrm{an}}}
\newcommand{\Pel}{P_\mathrm{el}}
\newcommand{\Pstr}{P_\mathrm{str}}
\newcommand{\Posm}{P_\mathrm{osm}}
\newcommand{\Pbox}{P_\mathrm{box}}
\newcommand{\Pext}{P_\mathrm{ext}}
\newcommand{\Req}{R_\mathrm{eq}}
\newcommand{\Veq}{V_\mathrm{eq}}
\newcommand{\Qeq}{Q_\mathrm{eq}}
\newcommand{\QV}{Q_{\mathrm{V}}}
\newcommand{\QR}{Q_{\mathrm{\Rend}}}
\newcommand{\Vbox}{V_\mathrm{box}}
\newcommand{\Vchain}{V_\mathrm{chain}}
\newcommand{\Pin}[0]{P_\mathrm{in}}

\newcommand{\Aall}{\mathrm{A}}
\newcommand{\HA}{\mathrm{HA}}
\newcommand{\Aminus}{\mathrm{A}^{-}}
\newcommand{\Clminus}{\mathrm{Cl}^{-}}
\newcommand{\Naplus}{\mathrm{Na}^{+}}
\newcommand{\Hplus}{\mathrm{H}^{+}}
\newcommand{\OHminus}{\mathrm{OH}^{-}}
\newcommand{\cHplus}{c_{\Hplus}}
\newcommand{\cref}{c^{\ominus}}
\newcommand{\muna}{\mu_\mathrm{Na}}
\newcommand{\mucl}{\mu_\mathrm{Cl}}
\newcommand{\muh}{\mu_\mathrm{H}}
\newcommand{\muoh}{\mu_\mathrm{OH}}
\newcommand{\cH}{\ensuremath{c_{\Hplus{}}}}
\newcommand{\cOH}{\ensuremath{c_{\OHminus{}}}}
\newcommand{\cNa}{\ensuremath{c_{\Naplus{}}}}
\newcommand{\cCl}{\ensuremath{c_{\Clminus{}}}}
\newcommand{\cA}{\ensuremath{c_{\ce{A-}}}}
\newcommand{\cHres}{\ensuremath{\cH\res{}}}
\newcommand{\cOHres}{\ensuremath{\cOH\res{}}}
\newcommand{\cNares}{\ensuremath{\cNa\res{}}}
\newcommand{\cClres}{\ensuremath{\cCl\res{}}}


\newcommand{\Vo}{V_\mathrm{0}}
\newcommand{\Vd}{V_\mathrm{d}}

\newcommand{\Van}{\overline{V}_\mathrm{an}}
\newcommand{\Vcat}{\overline{V}_\mathrm{cat}}
\newcommand{\Vs}{\overline{V}_\mathrm{s}}
\newcommand{\Vw}{\overline{V}_\mathrm{w}}
\newcommand{\Vm}{\overline{V}_\mathrm{m}}

\newcommand{\gel}{^{\mathrm{gel}}}
\newcommand{\res}{^{\mathrm{res}}}

\newcommand{\der}{\mathrm{d}} % for todal derivative
\newcommand{\Nav}{N_{\mathrm{A}}}
\newcommand{\nubar}{\bar{\nu}}


\newcommand{\Kw}{K_{\mathrm{w}}}
\newcommand{\pKw}{\mathrm{p}K_{\mathrm{w}}}
\newcommand{\pK}{\mathrm{p}K_\mathrm{A}}
\newcommand{\pH}{\mathrm{pH}}
\newcommand{\pHsys}{\pH\gel}
\newcommand{\pHres}{\pH\res}
\newcommand{\Ires}{I\res}

\newcommand{\pI}{\mathrm{p}\idp}
\newcommand{\pOH}{\mathrm{pOH}}

\newcommand{\es}{\textsc{ESPResSo}\xspace}
\newcommand{\ES}{\es}

\newcommand{\idp}{\ensuremath{I}}
\newcommand{\idpAB}{\ensuremath{\idp_{\sA{}\sB{}}}}
\newcommand{\idpAD}{\ensuremath{\idp_{\sA{}\sD{}}}}
\newcommand{\idpCB}{\ensuremath{\idp_{\sC{}\sB{}}}}
\newcommand{\idpCD}{\ensuremath{\idp_{\sC{}\sD{}}}}
\newcommand{\idps}{\ensuremath{\mathcal{I}^2}}
\newcommand{\idpsAB}{\ensuremath{\idps_{\sA{}\sB{}}}}
\newcommand{\idpsAD}{\ensuremath{\idps_{\sA{}\sD{}}}}
\newcommand{\idpsCB}{\ensuremath{\idps_{\sC{}\sB{}}}}
\newcommand{\idpsCD}{\ensuremath{\idps_{\sC{}\sD{}}}}

\newcommand*{\KNaCl}{K_{\mathrm{Na+Cl}}}
\newcommand*{\KHCl}{K_{\mathrm{H+Cl}}}
\newcommand*{\KNaOH}{K_{\mathrm{Na+OH}}}
\newcommand*{\KHNa}{K_{\mathrm{Na-H}}}
\newcommand*{\KOHCl}{K_{\mathrm{Cl-OH}}}
\newcommand*{\KHOH}{K_{\mathrm{H+OH}}}

% Figure and equation references
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\refsec}[1]{Section~\ref{#1}}
\newcommand{\refeq}[1]{Eq.~\ref{#1}}

\newcommand{\epsilonr}{\epsilon_\mathrm{r}}

% red strikeout
\usepackage[normalem]{ulem} % enables command \sout for strikeout
\newcommand{\soutr}[1]{\sout{\textcolor{red}{#1}}}
\newcommand{\soutb}[1]{\sout{\textcolor{blue}{#1}}}
% shorthand for my blue
\newcommand{\myblue}[1]{\textcolor{blue}{#1}}
\newcommand{\myred}[1]{\textcolor{red}{#1}}
% uncomment the line below to produce pdf in the final form, without the strikeouts and colours
\renewcommand{\soutr}[1]{\relax}
\renewcommand{\soutb}[1]{\relax} \renewcommand{\myblue}[1]{#1} \renewcommand{\myred}[1]{#1}


\usepackage{subcaption}
\captionsetup[subfigure]{list=true, font=large, labelfont=bf, 
labelformat=brace, position=top}

